Analyzing and Mitigating Inconsistency in Discrete Audio Tokens for Neural Codec Language Models

Building upon advancements in Large Language Models (LLMs), the field of audio processing has seen increased interest in training audio generation tasks with discrete audio token sequences. However, directly discretizing audio by neural audio codecs often results in sequences that fundamentally differ from text sequences. Unlike text, where text token sequences are deterministic, discrete audio tokens can exhibit significant variability based on contextual factors, while still producing perceptually identical audio segments. We refer to this phenomenon as \textbf{Discrete Representation Inconsistency (DRI)}. This inconsistency can lead to a single audio segment being represented by multiple divergent sequences, which creates confusion in neural codec language models and results in omissions and repetitions during speech generation. In this paper, we quantitatively analyze the DRI phenomenon within popular audio tokenizers such as EnCodec. Our approach effectively mitigates the DRI phenomenon of the neural audio codec. Furthermore, extensive experiments on the neural codec language model over LibriTTS and large-scale MLS datases (44,000 hours) demonstrate the effectiveness and generality of our method. The demo of audio samples is available online~\footnote{\url{https://consistencyinneuralcodec.github.io}}.

==> section/0_abstract.tex <==
% Building upon the advancements of large language models, the field of audio processing has seen increased interest in training audio generation tasks with discrete token sequences. However, directly discretizing audio often results in sequences that differ fundamentally from text sequences. Unlike text, where token sequences are deterministic, discrete acoustic tokens can exhibit significant variability based on contextual factors, such as silent segments at the end, while still producing perceptually identical speech segments. We refer to this phenomenon as Discrete Representation Inconsistency (DRI). It can result in a single audio segment being represented by multiple divergent sequences, leading to confusion in language models and subsequently causing omissions and repetitions in speech generation. In this paper, we quantitatively analyze DRI in popular audio tokenizers such as Encodec. We then propose methods to improve the audio tokenizer’s DRI by making the sequences consistent against contextual variations or noise perturbations in the audio input. Experimental results demonstrate that our approach significantly reduces inconsistency. Furthermore, our audio tokenizer is compatible with the VALLE language model. 


Building upon advancements in LLMs, the field of audio processing has seen increased interest in training audio generation tasks with discrete audio tokens sequences. However, directly discretizing audio by
neural audio codecs often results in sequences that fundamentally differ from text sequences. Unlike text, where token sequences are deterministic, discrete audio tokens can exhibit significant variability based on contextual factors, while still producing perceptually identical speech segments. We refer to this phenomenon as \textbf{Discrete Representation Inconsistency (DRI)}. This inconsistency can lead to a single audio segment being represented by multiple divergent sequences, which creates confusion in neural codec language models and results in omissions and repetitions during speech generation. In this paper, we quantitatively analyze DRI phenomenon within popular audio tokenizers such as EnCodec. Our approach effectively mitigates the DRI phenomenon of the neural audio codec. Furthermore, extensive experiments on the neural codec language model over LibriTTS and large-scale MLS English datases(~44k hours) demonstrate the generality and effectiveness of our method.

% significantly improving the performance of the neural codec language model VALLE for TTS tasks. Specifically, the WER decreases from 5.51\% to 3.85\%, and speaker similarity increases from 83.58\% to 87.24\%.


% We then propose consistent constraint methods to reduce the audio tokenizer’s DRI by making the sequences consistent against contextual variations or minor perturbations in the audio input. Experimental results demonstrate that our approach significantly reduces the DRI phenomenon of the audio tokenizer, and furthermore, improves the performance of the neural codec language model, VALLE, in TTS tasks. Specifically,  WER decreases from 5.51\% to 3.85\%, and speaker similarity increases from 83.58\% to 87.24\%. %Furthermore, our audio tokenizer is compatible with VALL-E.
% consistency increases from 12.21\% to 80.75\%,


% TTS models and multimodal LLMs can more effectively understand and generate audio by using neural audio codec as audio tokenizer, which convert continuous audio signals into discrete units. However, a \textbf{one-to-many} relationship exists within codecs, where the same audio signal may be converted into different acoustic representations. This inconsistency phenomenon complicates the learning process for neural codec language models, as they must map various representations back to the same audio signal. 
% Our quantitative analysis of the one-to-many relationship reveals that enforcing two specific consistencies in the neural audio codec can significantly reduce the one-to-many relationship, and improve neural codec language models' performance: 1) slice consistency: Audio segments with identical content should be encoded into consistent acoustic representations. 2) perturbation consistency: The acoustic representations of an audio signal should remain stable under minimal, imperceptible perturbations to human ears. Based on these findings, we propose a simple yet effective training method called \textbf{consistency constraints}, which improves the accuracy of the neural codec language models in predicting discrete units. Experimental results show that consistency constraints improve both the content accuracy (measured by WER) and speaker similarity of generated audio, resulting in improvements of 26.77\% and 3\%, respectively.

% enhance the training efficiency of downstream TTS models


==> section/1_introduction.tex <==
Recently, speech LLMs\citep{zhan2024anygpt, anastassiou2024seed, du2024cosyvoice} have demonstrated significant strides in generating high-quality speech, largely due to the contributions of neural audio codecs in high-fidelity audio reconstruction\citep{zeghidour2021soundstream, defossez2022high, yang2023hifi}. The neural codec language model\citep{VALL-E, yang2024uniaudio, zhang2024speechgpt} employs the neural audio codec as the audio tokenizer to quantize continuous audio signals into discrete units, and it can generate discrete units autoregressively\citep{zhang2023speechgpt, yang2024uniaudio}, and then detokenize them back into audio signals by the neural audio codec. Despite enjoying the advantages of autoregressive modeling, those works achieve better zero-shot performance and naturalness. However, the output speech frequently yields higher WER due to the issue of instability in codec generation\citep{song2024ella, xin2024rall, du2024vall}.

% Despite enjoying the advantages of autoregressive modeling, those works often achieve better prosody performance.

%VALL-E\citep{VALL-E} adopts EnCodec\citep{defossez2022high} as audio tokenizer to tokenize all acoustic representations, while SpeechGPT-gen\citep{zhang2024speechgpt} and AnyGPT\citep{zhan2024anygpt} utilize SpeechTokenizer\citep{zhang2023speechtokenizer} to encode speech into semantic and acoustic tokens. Each of them generates first layer of units autoregressively, and predicts remaining units in a non-autoregressive way. FACodec, employed in NaturalSpeech3\citep{ju2024naturalspeech}, decouples speech into phoneme, prosody, and timbre. This aids in the finely-tuned control of various speech attributes, ultimately leading to higher-quality audio generation. LanguageCodec\citep{ji2024language} seeks to preserve more acoustic details in deeper layer of units by masking codebooks' channels, leading to reduce the difficulty of units generation. 
% 太啰嗦，哪个Introduction写这么长以往的工作？？
% SpeechGPT-Gen\citep{zhang2024speechgpt} and AnyGPT\citep{zhan2024anygpt} utilize SpeechTokenizer\citep{zhang2023speechtokenizer} as their audio tokenizers to encode speech into both semantic tokens and acoustic tokens. This allows LLMs to model speech using only a layer of semantic tokens.
% \citep{kumar2024high, wu2023audiodec} focus on reconstructing high-fidelity audio, while some studies explore compressing audio at low bit rates\citep{jiang2023disentangled} and with fewer codebooks\citep{li2024single, liu2024semanticodec}. \citep{du2024funcodec, siuzdak2023vocos} also pay attention to features in both the time domain and frequency domain to achieve higher reconstruction quality.
% After the neural audio codec tokenizes the continuous audio signals into discrete units,


\begin{figure}[t]
  \centering
  % \includegraphics[width=1.0\textwidth]{figure/all_tokenizer.png}
  \includegraphics[width=1.0\textwidth]{figure/notion/all_tokenizer.png}
  \caption{\textbf{Discrete Representation Inconsistency (DRI) phenomenon} within audio tokenizers. \textbf{subfigure (a)}: a small slice of text is extracted from the source text, and tokens encoded by the BPE tokenizer are compared. Tokens in italics denote identical matches. \textbf{subfigure (b)}:  a small slice is extracted from the entire audio, and both of them are tokenized by the neural audio codec to obtain discrete units. After quantization, inconsistent units are indicated by varying colors at each layer of codewords. When comparing sub-figure (a) and (b), it is observed that identical words are consistently encoded into the same tokens by the text tokenizer, while identical audio segments are encoded into different units by the audio tokenizer. This highlights that DRI within the audio tokenizer poses a significant challenge for modeling discrete units.}
  \label{fig:all_tokenizer}
\end{figure}


% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1.0\textwidth]{figure/text_one_to_one.png}
%   \caption{\textbf{Consistency phenomenon} within text tokenizers. A small slice of text is extracted from the source text, and the tokens encoded by the BPE tokenizer are compared. Italics indicate that the tokens in the corresponding positions are the same.}
%   \label{fig:text_one_to_one}
% \end{figure}

% text离散化. 探究audio如何离散化
% 定量分析
% 降低in-consistency, 信息又足够的饱和
% 合并这两段
% 如何统计分析. 得出结果
% 3 items 
The discrete sequence of text is context-independent. In contrast, acoustic discrete representations are encoded by integrating the contextual information. The advantage of this approach is that discrete tokens consider a larger receptive field of information, thus achieving a higher compression ratio of information. However, the drawback is that the representation itself becomes more fragile and sensitive, easily affected by minor signal changes, leading to drastic drifts in the entire sequence as demonstrated in Figure~\ref{fig:all_tokenizer}.

% Text tokenizers typically employ BPE\citep{sennrich2015neural}, WordPiece\citep{schuster2012japanese}, or SentencePiece\citep{kudo2018sentencepiece} to split text into words or subwords. In contrast, acoustic discrete representation are encoded as codes by intergrating the contextual information. Neural audio codecs, served as audio tokenizers, utilize K-means\citep{lakhotia2021generative}\citep{lee2021textless} or Vector Quantization\citep{kharitonov2023speak}\citep{VALL-E} framework to map continuous audio signals into discrete units, referred as audio tokens, thereby enabling efficient audio encoding for neural codec language models. Text tokenizers and audio tokenizers adopt distinct tokenization approaches, resulting in tokens with different characteristics, particularly in terms of tokens' consistency. As shown in Figure \ref{fig:all_tokenizer} (a)(b), the tokens generated by the text tokenizer are context-independent, and the same text content is always encoded as the same token. This ensures tokens consistency when processing text. 

% \begin{wrapfigure}{l}{5.5cm}
%   \centering
%   \includegraphics[width=0.4\textwidth]{figure/curve/each_layer.png}
%   \caption{Consistency accuracy across each of the first 8 layers in neural audio codecs.}
%   \label{fig:each_layer_consistency}
% \end{wrapfigure}

The previous work~\citep{yang2024uniaudio} has noticed that audio segments containing the same sound events aren't encoded into completely consistent discrete acoustic tokens by the neural audio codec. In this paper, we call this phenomenon \textbf{Discrete Representation Inconsistency (DRI)}, and further dig into the problem on VQ-based acoustic tokens due to its popularity as an audio tokenizer and its high-quality reconstruction capabilities. We compare the consistency of the discrete sequences of audio segments with and without context on a large amount of audio. Our quantitative analyses reveal that existing tokenizers suffer from low consistency. In particular, we find that for residual VQ approaches, consistency declines significantly with deeper layers. 
%Through our quantitative analyses, we observe existing tokenizers suffer from low consistency as shown in Figure~\ref{fig:each_layer_consistency}. Especially, for residual VQ approaches, consistency drops rapidly as layers go deeper. %This reveals that discrete units derived from the first VQ layer are a little inconsistent, but DRI phenomenon becomes more pronounced in deeper VQ layers.
%As shown in in Figure \ref{fig:all_tokenizer} (b)(c), the neural audio codec encodes the same audio samples into different acoustic representations, resulting in different discrete units for the same audio samples. We call this phenomenon \textbf{Discrete Representation Inconsistency (DRI)}. 
%To conduct a quantitative analysis of the phenomenon, we employ accuracy as a metric to measure consistency among popular codecs. It is evident that consistency accuracy is inversely related to the DRI phenomenon, and lower consistency accuracy indicates more severe DRI phenomenon. As described in Figure \ref{fig:each_layer_consistency}, 
% consistency accuracy drops rapidly from the 1st VQ layer to the 8th VQ layer. This reveals that discrete units derived from the first VQ layer are a little inconsistent, but DRI phenomenon becomes more pronounced in deeper VQ layers.

% The DRI phenomenon presents challenges for neural codec language models in tokenizing the same audio samples into consistent discrete units. This reduces the model's accuracy in predicting discrete units, and directly impacts its performance on speech generation tasks. Therefore, it is essential to reduce the DRI phenomenon within neural audio codecs while maintaining their capacity to reconstruct high-fidelity audio.

% The DRI phenomenon presents challenges for neural codec language models in mapping the same audio samples into consistent discrete units. In the neural audio codec, the shallow layers of the RVQ contain more acoustic information, which gradually decreases in deeper layers\citep{liu2015improved}. Therefore, accurately predicting the discrete units within these shallow RVQ layers is vital for generating high-quality audio. If the shallow discrete units are inconsistent, the model will struggle to accurately extract and utilize the rich acoustic information they contain. This inconsistency can negatively impact processing in the subsequent VQ layers and ultimately affect the quality of the generated audio. Therefore, it is essential for speech generation task to reduce the DRI phenomenon within neural audio codecs while maintaining their capacity to reconstruct high-fidelity audio.

Since both audio with or without contextual audio can be encoded and used for reconstructing the original audio information. As a result, these discrete sequences poses a many-to-one mapping problem, and the complexity of this many-to-one mapping grows exponentially with the length of the discrete sequence. This complexity results in increased uncertainty for language models in predicting the next token. One direct approach to addressing this issue is to prevent the audio tokenizer from considering contextual information during sequence encoding, such as by setting the convolutional layer's kernel size to 1 of encoder. While this method allows for independent discretization of each audio frame, it also significantly reduces encoding efficiency and degrades the quality of the reconstructed audio. Therefore, this study aims to maintain the original receptive field while enabling the model to address the trade-offs between audio quality reconstruction and resolving the many-to-one problem. To achieve this objective, we introduce the \textbf{slice-consistency} method, wherein a segment of audio is randomly sliced, and the encoded representation for this segment is required to closely approximate the corresponding representation obtained for the entire audio. In addition, in order to further alleviate the issue of many-to-one mapping, we propose \textbf{perturbation-consistency} method, whereby the representation of a piece of audio and its representation after applying slight spectral perturbation should closely align. Compared to EnCodec~\citep{defossez2022high}, our method has shown an average consistency improvement of 17.15\%, 27.33\%, 42.71\%, and 41.1\% in the first layer, the first 3 layers, the first 8 layers, and the first 16 layers, respectively. Extensive experiments on the neural codec language model (i.e., VALL-E\citep{VALL-E}) on standard LibriTTS~\citep{zen2019libritts} and large-scale MLS~\citep{PratapMLS} datasets (44k hours) confirms that improving consistency results in better performance. Our contributions are summarized as below:

% we propose a simple but effective training method called \textbf{consistency constraint}. First, for each audio segment, we extract slice containing the same audio samples. Then, we constrain the encoder with slice consistency and perturbation consistency, ensuring consistency in both content and auditory perception. This consistency is chiefly manifested in two aspects: 1) Slice consistency: audio segments with the same content should be encoded into consistent acoustic representations. 2) Perturbation consistency: acoustic representations of the audio signals should remain stable and unchanged after being subjected to imperceptible minor perturbations to human ears. By preserving such consistency, discrete units would exhibit higher consistency, thereby improving the accuracy rate of neural codec language models in predicting discrete units. In summary, the main contributions of this paper are as follows:


\begin{itemize}
\item We observe the discrete representation inconsistency (DRI) problems and conduct quantitative analyses for various acoustic codecs. We find that existing acoustic tokenizers suffer from low consistency.

\item Inspired by our analyses, we propose two methods, slice-consistency and perturbation-consistency, to mitigate the many-to-one issues. 

% \item Experiments shows that our method achieves an average consistency improvement of 17.15\%, 27.33\%, 42.71\%, and 41.1\% in the first layer, the first 3 layers, the first 8 layers, and the first 16 layers, respectively. Furthure, based on VALL-E, our proposed audio tokenizers achieves 47.37\% relative WER reduction and 7.31\% speaker similarity improvement on standard LibriTTS dataset. Trained with the large-scale MLS dataset, our methods shows up to 30.13\% relative WER reduction and 3.66\% speaker similarity improvement.

\item Experiments show that our method achieves an average consistency improvement of 17.15\%, 27.33\%, 42.71\%, and 41.1\% in the first layer, the first 3 layers, the first 8 layers, and the first 16 layers, respectively. Furthure, based on VALL-E\citep{VALL-E}, our proposed audio tokenizers achieves 6.20\% WER reduction and 7.31\% speaker similarity improvement on standard LibriTTS\citep{zen2019libritts} dataset. Trained on
the large-scale MLS\citep{PratapMLS} dataset with 44k hours of English, our methods shows up to 2.69\% WER reduction and 2.32\% speaker similarity improvement.

\end{itemize}


% Experimental results demonstrate that the consistency constraint achieves higher consistency across various neural audio codec configurations, leading significant improvements in WER, speaker similarity and naturalness in neural codec language models.


==> section/2_analyze_consistency.tex <==
% \begin{figure}[htbp]
%     \centering
%     \subfloat[all layers]{\includegraphics[scale=0.366]{figure/curve/all_layers.png}\label{fig:subfig1}}
%     \hfill
%     \subfloat[the first 3 layers]{\includegraphics[scale=0.366]{figure/curve/3_layers.png}\label{fig:subfig2}}
%     \hfill
%     \subfloat[the first 8 layers]{\includegraphics[scale=0.366]{figure/curve/8_layers.png}\label{fig:subfig3}}
%     \caption{Results of consistency accuracy for popular neural audio codecs under various slice lengths. Sub-figure (a)(b)(c) show consistency accuracy across \textbf{all layers}, \textbf{the first 3 layers}, \textbf{the first 8 layers} within neural audio codecs, respectively. The slice lengths range from 0.2s to 4.0s, demonstrating the consistency of each codec across different temporal granularities and context lengths.}
%     \label{fig:analysis_on_consistency}
% \end{figure}


\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\textwidth]{figure/notion/8_layer_fig.png}
  %\caption{Results of consistency accuracy for different neural audio codecs under various slice lengths. Sub-figure (a)(b)(c) show slice lengths across 0.2s, 0.3s, 0.4s respectively, and longer slice lengths demonstrates more context information is introduced when neural audio codec encodes audio into discrete units. The consistency accuracy declines significantly in deeper layers of the codebook, indicating that the \textbf{DRI} phenomenon becomes more pronounced.}
    \caption{Results of consistency accuracy for popular neural audio codecs under various layers and various slice lengths. Sub-figure (a)(b)(c) show slice lengths across 0.2s, 0.3s, 0.4s respectively, and all of them exhibit similar conclusions that consistency accuracy declines significantly in the deeper layers of the codebook, indicating that the DRI phenomenon becomes more pronounced with the receptive field of the convolutional layers in neural audio codecs increasing.}
  \label{fig:analysis_on_consistency}
\end{figure}


% \begin{table}[!ht]
%     \centering
%     \caption{Zero-shot TTS evaluation results of neural codec language models. Codecs with different consistency accuracy are used as audio tokenizers to map audio samples into discrete units.}
%     \scalebox{0.9}{
%     \begin{tabular}{cc|cc|ccc}
%     \toprule
%         consistency & \makecell[c]{first 3 layers'\\ consistency} & \makecell[c]{top 10\\ prediction accuracy} & \makecell[c]{prediction \\ accuracy} & WER↓ & SIM↑ & UTMOS↑ \\ 
%         \toprule
%         11.87\% & 23.92\% & 65.1\% & 24.7\% & 13.11 & 79.61\% & 4.12 \\ \midrule
%         84.44\% & 94.63\% & 69.8\% & 26.2\% & 9.13 & 83.77\% & 4.15 \\ \midrule
%         86.38\% & 95.77\% & 72.4\% & 28.4\% & 6.90 & 86.92\% & 4.32 \\
%     \bottomrule
%     \label{consistency_for_tts}
%     \end{tabular}
%     }
% \end{table}



% In this section, we first discuss the inherent \textbf{DRI phenomenon} within neural audio codecs as well as its potential impacts on downstream neural codec language models. Subsequently, we introduce the \textbf{consistency accuracy} as a metric to measure the DRI phenomenon. 

%In this section, we first construct a pair of audio signals containing identical content, and investigate whether a neural audio codec encodes them into inconsistent discrete acoustic units. Subsequently, we introduce the \textbf{consistency accuracy} as a metric to measure the DRI phenomenon. At last, we examine the existence of the DRI phenomenon in neural audio codecs, and discuss its potential impacts on downstream neural codec language models.


In this section, we extract discrete unit sequences of audio segments with and without context using popular neural audio codecs~\citep{defossez2022high, yang2023hifi, zhang2023speechtokenizer, du2024funcodec, kumar2024high, ju2024naturalspeech} to analyze the DRI phenomenon in neural audio codecs. To demonstrate that current neural audio codecs exhibit low consistency, we propose using \textbf{consistency accuracy} as an evaluation metric and assess the potential implications of the DRI phenomenon.

% EnCodec defossez2022high
% SoundStream zeghidour2021soundstream
% HiFigan yang2023hifi
% SpeechTokenizer zhang2023speechtokenizer
% FunCodec du2024funcodec
% DAC kumar2024high
% FACodec ju2024naturalspeech

% \subsection{Neural audio codec}

% A continuous audio signal can be represented as $X \in \mathbb{R}^{C \times T}$, where $C$ is the number of audio channels, and $T$ is the number of frames. A neural audio codec is typically composed of four components: an encoder $E$, a residual vector quantizer $Q$, a decoder $G$, and a discriminator $D$. For the purpose of this discussion, we simplify the number of audio channels $C$ to one.
% an encoder $E$, a residual vector quantizer $Q$, a decoder $G$, and a discriminator $D$

% Neural audio codecs employ the RVQ framework to compress continuous audio signals into discrete units. A neural audio codec is typically composed of four components: (1) The encoder $E$ initially maps audio signal $X^{T}$ into a latent vector $Z^{\frac{T}{f_{ds}}}$, with $f_{ds}$ denoting the downsampling rate of the encoder. (2) The quantizer maps $Z^{\frac{T}{f_{ds}}}$ onto the nearest codebook embedding based on Euclidean distance, yielding the quantized $E^{\frac{T}{f_{ds}}}$. (3) The decoder $D$ reconstructs the original audio $\hat{X}$ from the quantized $E^{\frac{T}{f_{ds}}}$. (4) In the training process, the discriminator's role is to discern whether audio samples are real or reconstructed. 

% with the objective of minimizing the perceptual differences between the reconstructed and original audio

% \subsection{Experiment design on DRI phenomenon}
% Experiment analysis

% \begin{figure}
%   \centering
%   \includegraphics[width=.8\textwidth]{figure/model.jpg}
%   \caption{model,草稿}
%   \label{model}
% \end{figure}

% 直观的引导. 省略公式
% In this subsection, we construct a pair of audio signals containing identical content. The goal is to investigate whether a neural audio codec might encode them into varying discrete acoustic units when processing audio signals with the same content. In other words, we examine whether a single audio segment could correspond to multiple acoustic representations.
% Specifically, given an audio signal $X_1 = [x_1, \ldots, x_{t}]$, we produce a segment $X_2 = [x_{t_s}, \ldots, x_{t_e}]$ by selecting audio samples within the time interval $I_t = [t_s, t_e]$ from $X_1$. That is, $X_2$ is a subsequence of the original audio signal $X_1$ within $I_t$. We refer to this operation as slicing in the time domain, denoted $S_t$, expressed as:
% $$X_2 = S_t(X_1) = \{x_i \mid x_i \in X_1, t_s \leq i \leq t_e\}$$
% The encoder maps $X_1$ and $X_2$ into latent vectors $Z_1 = [z_1, \ldots, z_{\frac{t}{f_{ds}}}]$ and $Z_2 = [z_{\frac{t_s}{f_{ds}}}, \ldots, z_{\frac{t_e}{f_{ds}}}]$, respectively. The quantizer then quantizes these latent vectors into sequences of discrete acoustic units, $E_1 = [e_1, \ldots, e_{\frac{t}{f_{ds}}}]$ and $E_2 = [e_{\frac{t_s}{f_{ds}}}, \ldots, e_{\frac{t_e}{f_{ds}}}]$. After being downsampled by a factor of $f_{ds}$ by the encoder, the chosen audio samples within the time interval $I_t$ correspond to the feature interval $I_f = [\frac{t_s}{f_{ds}}, \frac{t_e}{f_{ds}}]$. By extracting the subsequence within the feature interval $I_f$ from $Z_1$ and $E_1$, we obtain $\tilde{Z}_1$ and $\tilde{E}_1$. Notably, the boundaries of the selected audio interval, $t_s$ and $t_e$, are multiples of $f_{ds}$ to avoid temporal misalignment between $Z_2$ and $\tilde{Z}_1$. This operation, slicing on the feature sequence, is denoted as $S_f$, and defined as:
% $$\tilde{Z}_1 = S_f(Z_1) = \{z_i \mid z_i \in Z_1, \frac{t_s}{f_{ds}} \leq i \leq \frac{t_e}{f_{ds}}\}$$
% $$\tilde{E}_1 = S_f(E_1) = \{e_i \mid e_i \in E_1, \frac{t_s}{f_{ds}} \leq i \leq \frac{t_e}{f_{ds}}\}$$
% Clearly, $\tilde{Z}_1$ and $Z_2$ encode the same audio samples. Intuitively, we would expect that after processing through the quantizer, the discrete unit sequences $\tilde{E}_1$ and $E_2$ should be identical. However, the presence of convolutional layers in the encoder allows $\tilde{Z}_1$ to capture features from other audio samples within its receptive field. As a result, despite $\tilde{Z}_1$ and $Z_2$ encoding the same audio content, $\tilde{E}_1$ and $E_2$ exhibit significant divergences, giving rise to the DRI phenomenon. This implies that the same audio content, once encoded, corresponds to disparate acoustic representations, thereby complicating the prediction for downstream neural codec language models.
% Additionally, operations such as layer normalization or time-group normalization integrate global features into $\tilde{Z}_1$, endowing it with additional audio information compared to $Z_2$. 

\subsection{Experimental design on DRI phenomenon}
% In this subsection, we construct a pair of audio signals containing identical content, to investigate whether a neural audio codec encodes them into inconsistent discrete acoustic units. Our goal is to examine the existence of the DRI phenomenon in neural audio codecs.

% Neural audio codecs employ the RVQ framework to compress continuous audio signals into discrete units. A neural audio codec is typically composed of four components: (1) The encoder $E$ initially maps audio signal $X^{T}$ into a latent vector $Z^{\frac{T}{f_{ds}}}$, with $f_{ds}$ denoting the downsampling rate of the encoder. (2) The residual vector quantizer $Q$ maps $Z^{\frac{T}{f_{ds}}}$ onto the nearest codebook embedding based on Euclidean distance, yielding the quantized $E^{\frac{T}{f_{ds}}}$. (3) The decoder $D$ reconstructs the original audio $\hat{X}$ from the quantized $E^{\frac{T}{f_{ds}}}$. (4) In the training process, the discriminator's role is to discern whether the audio is real or reconstructed. 

Recent advancements on neural audio codecs have adopted an encoder-decoder architecture combined with RVQ to effectively compress continuous audio signals into discrete tokens~\citep{defossez2022high, yang2023hifi, zhang2023speechtokenizer, du2024funcodec, kumar2024high, ju2024naturalspeech}, which is typically composed of three components: (1) an encoder initially maps audio signal into a latent representation $Z$; (2) a RVQ typically contains $N$ quantization layers, hence at each time step to maps latent representation $Z$ into the discrete audio tokens; (3) a decoder reconstructs the audio from the quantized latent representation. To analyze the inconsistency of discrete audio tokens quantized by different neural audio codecs, as shown in Figure~\ref{fig:all_tokenizer} (b), we use existing neural audio codecs~\citep{defossez2022high, yang2023hifi, zhang2023speechtokenizer, du2024funcodec, kumar2024high, ju2024naturalspeech} to quantize both the complete audio and an audio segment within that audio, and then compare the results of their corresponding discrete audio tokens.

Intuitively, these two audio segments are exactly the same with the only difference being whether there is context, and we would expect that both discrete audio tokens should be identical after the quantification. However, considering reconstruction efficiency and quality, convolutional layers are typically used in the encoders~\citep{defossez2022high, yang2023hifi, zhang2023speechtokenizer, du2024funcodec, kumar2024high, ju2024naturalspeech} to capture contextual information within the receptive fields. As a result, these two discrete audio tokens show significant differences, giving rise to the DRI phenomenon. 

%we would expect that after processing through the quantizer, discrete unit sequences $\tilde{E}_1$ and $E_2$ should be identical. However, the presence of convolutional layers in the encoder allows $\tilde{Z}_1$ to capture contextual information from other audio segments within its receptive field. As a result, despite $\tilde{Z}_1$ and $Z_2$ encoding the same audio content, $\tilde{E}_1$ and $E_2$ exhibit significant divergences, giving rise to the DRI phenomenon. 

%As shown in Figure \ref{fig:all_tokenizer} (d), given an audio signal $X_1 = [x_1, \ldots, x_{t}]$, we produce a segment $X_2 = [x_{t_s}, \ldots, x_{t_e}]$ by selecting audio segments within the time interval $I_t = [t_s, t_e]$ from $X_1$. That is, $X_2$ is a subsequence of the original audio signal $X_1$ within $I_t$. We refer to this operation as slicing in the time domain, denoted as $S_t$.

%As described in Figure \ref{fig:all_tokenizer} (e), the encoder maps $X_1$ and $X_2$ into latent vectors $Z_1$ and $Z_2$, respectively. The RVQ module then quantizes $Z_1$ and $Z_2$ into discrete unit sequences $E_1$ and $E_2$. After being downsampled by a factor of $f_{ds}$ by the encoder, the chosen audio segments within the time interval $I_t$ correspond to the feature interval $I_f = [\frac{t_s}{f_{ds}}, \frac{t_e}{f_{ds}}]$. By extracting the subsequence within the feature interval $I_f$ from $Z_1$ and $E_1$, we obtain $\tilde{Z}_1$ and $\tilde{E}_1$. Notably, the boundaries of the selected audio segments interval, $t_s$ and $t_e$, are multiples of $f_{ds}$ to avoid temporal misalignment between $Z_2$ and $\tilde{Z}_1$. This operation, slicing on the feature sequence, is denoted as $S_f$.

%In Figure \ref{fig:all_tokenizer} (d), $X_1$ and $X_2$ represent the audio segments in the upper and lower parts of subfigure (d), respectively. In Figure \ref{fig:all_tokenizer} (e), $Z_1$ and $Z_2$ denote the discrete units in the upper and lower parts of subfigure (e), respectively, while $\tilde{Z}_1$ indicates the shaded discrete units in the upper part of subfigure (e).

%Clearly, $\tilde{Z}_1$ and $Z_2$ are encoded from the same audio segments. Intuitively, we would expect that after processing through the quantizer, discrete unit sequences $\tilde{E}_1$ and $E_2$ should be identical. However, the presence of convolutional layers in the encoder allows $\tilde{Z}_1$ to capture contextual information from other audio segments within its receptive field. As a result, despite $\tilde{Z}_1$ and $Z_2$ encoding the same audio content, $\tilde{E}_1$ and $E_2$ exhibit significant divergences, giving rise to the DRI phenomenon. 

% This implies that the same audio content, once encoded, corresponds to disparate acoustic representations, thereby complicating the prediction for downstream neural codec language models.

\subsection{Consistency accuracy}
% high level. 不用具体数值解释 (top10-acc)
%We quantify the degree of the \textbf{DRI phenomenon} in the neural audio codec, by calculating the consistency accuracy between the sequences of discrete units $ \tilde{E}_1 $ and $ E_2 $, defined as:
%$$acc_{\text{consistency}} = \frac{1}{T} \sum_{t=1}^{T} \sum_{i=1}^{N} \mathbb{I}(\tilde{E}_1[t, i] = E_2[t, i])$$
%where $ T $ represents the length of discrete unit sequences $E_2$, and is equal to $\lfloor (t_e - t_s) / f_{ds} \rfloor$. $ N $ represents the number of codebooks, and $ \mathbb{I}\{\cdot\} $ is the indicator function. That is, $ \mathbb{I}(\cdot)=1 $ if the condition is true; otherwise, $ \mathbb{I}(\cdot)=0 $. Figure \ref{fig:analysis_on_consistency} shows the consistency accuracy of popular codecs, specifically considering the consistency accuracy under various slice length. The slice length is equal to $t_e - t_s$.
% The measure of consistency $ acc_{\text{consistency}} $ is inversely correlated with the \textbf{DRI phenomenon} relationship: a higher value of consistency accuracy indicates a less pronounced DRI phenomenon issue; a lower consistency accuracy suggests a more significant one-to-many relationship. 

% As Figure \ref{fig:analysis_on_consistency} shows, we analyze the consistency accuracy of mainstream codecs, specifically considering the consistency accuracy across all layers, the first 3 layers, and the first 8 layers. The values of $N$ are the number of codebooks in the codec, 3, and 8, respectively. HiFiCodec only has 4 codebooks, so when calculating the consistency of more than 4 layers for HiFiCodec, it is essentially equivalent to the consistency of its first 4 layers.

To quantitatively analyze the degree of the DRI phenomenon in neural audio codecs, we propose using \textbf{consistency accuracy} as an evaluation metric:

% $$acc_{\text{consistency}} = \frac{1}{T} \sum_{t=1}^{T} \sum_{i=1}^{N} \mathbb{I}(\tilde{E}_1[t, i] = E_2[t, i])$$

$$Acc_{\text{consistency}} = \frac{1}{T} \sum_{t=1}^{T} \sum_{i=1}^{N} \mathbb{I}(\text{RVQ}(Z^{slice})[t, i] = \text{RVQ}(Z)[t, i]),$$

% $$Acc_{\text{consistency}} = \frac{1}{T} \sum_{t=1}^{T} \sum_{i=1}^{N} \mathbb{I}(\text{RVQ}(Z^{t_s: t_e}_{t})[i] = \text{RVQ}(Z^{slice}_{t})[ i])$$,

where $Z$ is the latent representation of the original audio after encoding by the encoder, and $N$ represents the number of codebooks in the RVQ module. We randomly extract an audio segment of length $T$ from the original audio, and encode it by the encoder to obtain $Z^{slice}$.

% where $Z$ is the latent representation of the original audio after encoding by the encoder, and $N$ represents the number of codebooks in the RVQ module. We randomly extract an audio segment of length $T$ from the original audio within the time interval $[t_s, t_e]$, and encode it by the encoder to obtain $Z^{slice}$.


% The characteristics of these consistency metrics are described as follows:

% \textbf{Consistency across all layers}. This metric reflects the overall consistency of the codec. Notably, the consistency significantly drops at deeper layers. If only the first few layers are used as the audio tokenizer for the neural codec language model, this metric may not be fair.

% \textbf{Consistency of the first 3 layers}. In the RVQ framework, codewords in the first few layers contain more semantic and acoustic information. Therefore, to ensure accurate generation of audio content and acoustic attributes like timbre, the neural codec language model needs to precisely predict the discrete acoustic units in these first few layers. We evaluate the consistency of the first 3 layers to determine if it can help the neural codec language model learn more effectively.

% \textbf{Consistency of the first 8 layers}. We utilize the neural audio codec with 8 codebooks as the audio tokenizer for the neural codec language model, thus we study the consistency of the first 8 layers of the codec.

% HiFiCodec only has 4 codebooks. Hence, when calculating the consistency of more than 4 layers for HiFiCodec, it is essentially equivalent to the consistency of its first 4 layers.


\subsection{results and analysis}
%\textbf{Audio tokenizer vs. text tokenizer}. As shown in Figure~\ref{fig:all_tokenizer} (a)(b), when two slices of text containing the same words are encoded by a text tokenizer, the same text slices are tokenized into identical tokens. During the detokenization process, the same tokens are mapped back to identical text, creating a one-to-one relationship between text and tokens. However, when using a neural audio codec as audio tokenizer to process audio, even if the audio segments are identical, the codec may tokenize the same audio segments into different discrete units, as demonstrated in Figure \ref{fig:all_tokenizer} (d)(e). In other words, there is the one-to-many relationship between audio and tokens, leading to DRI phenomenon within neural audio codecs.

\textbf{Audio tokenizer vs. text tokenizer}. As shown in Figure~\ref{fig:all_tokenizer} (a), regardless of whether context is included, the same text is tokenized into the same tokens, indicating that text tokenizer is context-independent. In contrast, as shown in Figure~\ref{fig:all_tokenizer} (b), using a neural audio codec as the audio tokenizer may produce different discrete tokens for identical audio segments. This context dependence in neural audio codecs can make the representation itself more fragile and sensitive, rendering it easily affected by minor signal changes, which may lead to significant drifts in the entire sequence.

%\textbf{The reason for DRI within codecs}. This DRI phenomenon is mainly due to the encoder in the codec leveraging convolution layers to downsample the audio segments. The receptive field of the convolution layers capture contextual information, causing identical audio segments to be tokenized into different discrete units under varying contexts. Table \ref{receptive_field} in the appendix shows the receptive field sizes for each layer of the codec's encoder. During the process of encoding audio segments into discrete units, a segment of audio segments will be affected by adjacent 2718 audio segments.

%\textbf{The reason for DRI phenomenon within codecs}. The DRI phenomenon is mainly due to the encoder in the codec leveraging convolution layers to downsample the audio segments. The receptive field of the convolution layers capture contextual information, causing identical audio segments to be tokenized into different discrete tokens. Table \ref{receptive_field} in the appendix shows the receptive field sizes for each layer of the codec's encoder. During the process of encoding audio segments into discrete units, a segment of audio segments will be affected by adjacent 2718 audio segments.

\textbf{The reason for DRI phenomenon within codecs}. The encoder in the codec typically uses convolutional layers to downsample audio segments, and the receptive field of these convolutional layers captures contextual information, causing identical audio segments to be tokenized into different discrete tokens. However, reducing the kernel size of the convolutional layers in the encoder may result in a decline in both reconstruction efficiency and quality. Therefore, this study aims to preserve the original receptive field while allowing the model to address the trade-offs between audio quality reconstruction and addressing the many-to-one problem.

%\textbf{The trend of changes in consistency accuracy}. As illustrated in Figure \ref{fig:analysis_on_consistency}, there are inconsistent issue within the popular neural codecs like EnCodec\citep{defossez2022high} and HiFiCodec\citep{yang2023hifi}, primarily manifested in: 1) Neural audio codecs suffer lower consistency in deeper layers of codebooks. This means that the many-to-one phenomenon becomes increasingly pronounced in deeper layers. 2) The slice length also affects the consistency accuracy. When the slice length becomes longer, the codec encoder processes a longer audio segment, providing more contextual information that enables the model to capture long-term dependencies, which enhances consistency and reduces the DRI phenomenon. The DRI phenomenon poses challenges for neural codec language models in mapping audio segments to consistent discrete units, especially in predicting discrete units.

\textbf{The trend of changes in consistency accuracy}.  As shown in Figure~\ref{fig:analysis_on_consistency}, we calculated the consistency accuracy across different layers and slice lengths. We observe that the DRI phenomenon exists in the current neural audio codecs, which poses challenges for neural codec language models in mapping audio segments to consistent discrete audio tokens, especially in predicting discrete tokens. Furthermore, we find that with deeper layers of codebooks, neural audio codecs demonstrate lower consistency at different slice lengths, which demonstrates that the receptive field sizes of the convolutional layers increase as the number of layers increases (as shown in Appendix~\ref{analysis_inconsistencies}), leading to more contextual information and lower consistency.

% particularly in the shallow layers of the RVQ, which contain important acoustic information crucial for generating high-quality audio.

% \textbf{How consistency affects neural codec language models}? As shown in Table \ref{consistency_for_tts}, the accuracy of predicting discrete units by the neural codec language model increases with the rise in codec consistency, thereby enhancing the quality of generated audio. There are evident improvements in speech content (measured by WER), speaker similarity (measured by SIM), and naturalness (measured by UTMOS). This suggests that when the consistency of the codec becomes higher, the neural codec language model can more effectively learn the mapping relationship between audio and units, leading to more accurate predictions of discrete units.

% \textbf{How the DRI phenomenon affects neural codec language models}? The DRI phenomenon presents challenges for neural codec language models in mapping the same audio samples into consistent discrete units. In the neural audio codec, the shallow layers of the RVQ contain more acoustic information, which gradually decreases in deeper layers\citep{liu2015improved}. Therefore, accurately predicting the discrete units within these shallow RVQ layers is vital for generating high-quality audio. If the shallow discrete units are inconsistent, the model will struggle to accurately extract and utilize the rich acoustic information they contain. This inconsistency can negatively impact processing in the subsequent VQ layers and ultimately affect the quality of the generated audio. 


==> section/3_method.tex <==
% \subsection{1 Overview}

% Neural audio codecs employ the RVQ framework to encode continuous audio signals into discrete latent spaces, followed by quantization into a series of discrete acoustic units, and then reconstructing the original audio to facilitate audio compression. These discrete units enable various TTS models and multimodal LLMs to understand and generate audio more effectively. A significant challenge faced by neural audio codecs is the one-to-many relationship, where the same audio content could be discretized into different representations, thus increasing the complexity of learning discrete acoustic units for subsequent neural codec language model.

% We posit that an ideal neural audio codec should avoid the \textbf{one-to-many} relationship and maintain the \textbf{consistency} of acoustic representations. This consistency is chiefly manifested in two aspects: 1) Slice consistency: audio segments with the same content should be encoded into consistent acoustic representations. 2) Perturbation consistency: acoustic representations of the audio signals should remain stable and unchanged after being subjected to imperceptible minor perturbations to human ears. By preserving such consistency, the resulting discrete acoustic units would exhibit higher regularity, thereby improving the accuracy rate of neural codec language models in predicting discrete acoustic units, as well as improving the authenticity of the generated audio content and speaker timbre similarity.

\begin{figure}[t]
  \centering
  % \includegraphics[width=1.0\textwidth]{figure/model.png}
  \includegraphics[width=1.0\textwidth]{figure/notion/model.png}
  \caption{The overview of the proposed method. For the slice-consistency method, a segment of audio is randomly sliced, and its encoded representation must closely match the representation derived from the entire audio. For the perturbation-consistency method, the representation of a piece of audio and its representation after slight spectral perturbation should be closely aligned. }
  \label{fig:model}
\end{figure}

%  After applying imperceptible perturbations to the original audio, we extract a small slice from the perturbed audio. This small slice and the entire audio are then encoded by the neural audio codec, resulting in their respective acoustic features. During training, we enforce consistency constraints on these acoustic features.}

% \subsection{1 简化的Overview}

% \subsection{Consistency Learning}

%According to the analysis in Section~\ref{sec:analysis}, we can draw a conclusion that an ideal neural audio codec should avoid the \textbf{DRI phenomenon} and maintain the \textbf{consistency} of acoustic representations. As shown in Figure \ref{fig:model}, we propose a simple but effective method, called \textbf{consistency constraint}, to enhance the neural audio codec from two particular perspectives:


According to the analysis in Section~\ref{sec:analysis}, we can draw a conclusion that an ideal neural audio codec should balance the trade-offs between high audio quality reconstruction and the many-to-one problem. To achieve this objective, we introduce two methods: \textbf{slice-consistency} and \textbf{perturbation-consistency}, which enhance the neural audio codec from two particular perspectives. Since these methods can be integrated into any neural audio codec,  we demonstrate their application using a neural audio codec based on RVQ, which utilizes an encoder to transform the audio signals into the latent representation $Z$ and reconstructs waveform from the quantized latent representation $Z$.

%As shown in Figure~\ref{fig:model}, to achieve this objective, we first employ an encoder in the neural audio codec to convert audio signal into a latent representation $Z$, and then we introduce the \textbf{slice-consistency} and \textbf{perturbation-consistency} method to enhance the neural audio codec from two particular perspectives.

\subsection{Consistency Enhancement Methods}

\textbf{Slice-consistency}: as shown in Figure~\ref{fig:model}, we cut a segment of audio from the original audio, and then encode it using the same encoder in the neural audio codec to obtain the latent representation $Z^{slice}$. Compared with the latent representation $Z$ from the entire audio, $Z^{slice}$ is not influenced by contextual information. To reduce the influence of context on the latent representation $Z$ and enhance its consistency,  we use Mean Squared Error (MSE) as a constraint to enforce consistency between $Z^{slice}$ and the corresponding latent representations in $Z$: 

$$\mathcal{L}_\text{slice} =  \frac{1}{T} \sum_{t=1}^{T} \text{MSE}(Z^{slice}[t], Z[t]).$$

%1) Slice Consistency: Acoustic representations $\tilde{Z}_1$ and $Z_2$, which encode the same audio content, should be close to each other, so that the discrete unit sequences $\tilde{E}_1$ and $E_2$ resulting from the quantizer can remain consistent. Specifically, given an audio signal $X_1 = [x_1, \ldots, x_{t}]$, we randomly select a time interval $I_t = [t_s, t_e]$, and crop the audio within this interval to generate a new audio segment $X_2 = [x_{t_s}, \ldots, x_{t_e}]$. Subsequently, the encoder $E$ maps $X_1$ and $X_2$ to latent vectors $Z_1$ and $Z_2$. Clearly, the subsequence $\tilde{Z}_1$ of $Z_1$ over the feature interval $I_f = [\frac{t_s}{f_{ds}}, \frac{t_e}{f_{ds}}]$ encodes the same audio segments as $Z_2$. To enforce consistency between $ \tilde{Z}_1 $ and $ Z_2 $, we use Mean Squared Error as a constraint, denoted as
%$$loss_\text{slice} = \text{MSE}(\tilde{Z}_1, Z_2)$$

%2) Perturbation Consistency: The new audio signal $ X^*_1 $ obtained after subjecting the original audio signal $ X_1 $ to imperceptible slight perturbations $ P $ should be perceptually similar to $ X_1 $. The perturbation $ P $ can be applied through various methods, such slightly adjusting the phase of the audio signal without significantly altering the waveform structure. As human ears have limited direct perception of phase changes, such alterations are typically hard to detect. We also utilize MSE to constrain the encoded representations before and after perturbation, as follows:
%$$X^*_1 = P(X_1)$$
%$$loss_\text{perception} = \text{MSE}(E(X_1), E(X^*_1))$$

\textbf{Perturbation-Consistency}: as shown in Figure~\ref{fig:model}, we slightly adjust the phase of the the original audio without significantly altering the waveform structure, and encode it using the same encoder in the neural audio codec to obtain the latent representation $Z^{perception}$. Since human ears have a limited ability to directly perceive phase changes, we hope that the robustness of the model can also eliminate inconsistency caused by such slight perturbations. Therefore, we utilize MSE to maintain consistency of the latent representations with and without phase perturbation~\citep{phaseaug}:

$$\mathcal{L}_\text{perception} = \text{MSE}(Z^{perception}, Z).$$

It is evident that the perturbation consistency constraint differs from audio-based data augmentation methods. Data augmentation methods such as SpecAugment~\citep{park2019specaugment} and environment noise~\citep{snyder2015musan} significantly alter the original audio to create new audio. The newly generated audio has a considerable difference in perception compared to the original audio, which aims to expand the training data and increase the robustness of models. In contrast, the perception-consistency method requires that changes to audio should be imperceptible to human ears to avoid severe perturbations that disrupt the reconstruction quality of the neural audio codec. Since the phase is difficult to be perceived by human, we introduce phase perturbation~\citep{phaseaug} as a slight perturbation, which can enhance the perturbation consistency without expanding the training data.

\subsection{Implementation Details}

%Therefore, we introduce phase perturbation~\citep{phaseaug} as 

%, and therefore does not create new audio segments. Phase perturbation~\citep{phaseaug} fulfills this requirement, as the phase is difficult to be perceived by human. Therefore, phase perturbation is adopted to enhance the perturbation consistency within neural audio codecs.


%These newly generated audio data has a considerable difference in perception compared to the original audio. Data augmentation is commonly used to improve the stability and generalization of models. 

In order to satisfy both slice and perturbation consistency and enhance training efficiency, we enforce consistency between
the latent representation $Z^{perception}$ obtained by the slice-consistency method and the latent representation $Z^{perception}$ obtained by the perturbation-consistency method:

$$\mathcal{L}_\text{consistency} =  \frac{1}{T} \sum_{t=1}^{T} \text{MSE}(Z^{slice}[t], Z^{perception}[t]).$$

% We contend that an ideal neural audio codec should satisfy both slice and perturbation consistency, meaning the introduction of contextual information and slight perturbations should not affect the acoustic representation and discrete units. We enforce the perturbed representation $ E(X^*_1) $ over feature interval $ I_f = [\frac{t_s}{f_{ds}}, \frac{t_e}{f_{ds}}] $ to remain close to $ Z_2 $ to realize the consistency constraint. Specifically, for an audio signal $ X $, we apply slice and perturbation consistency constraints by
%$$loss_\text{consistency} = \text{MSE}(S_f \circ E \circ P(X), E \circ S_t(X))$$.
% \subsection{Training Object}


%The proposed method, called \textbf{consistency constraint}, is built on the RVQ-GAN framework\citep{du2024funcodec}. The overall training objective consists of five components: reconstruction loss, adversarial loss, feature matching loss, the RVQ commit loss, and the consistency loss, which are as follows:

In addition to this, our methods is built on RVQ-GAN framework~reconstruction loss, adversarial loss, feature matching loss, the RVQ commit loss, and the consistency loss and also include reconstruction loss, adversarial loss, feature matching loss, and commit loss:
$$
\mathcal{L} = \mathcal{L}_{\mathrm{rec}} + \lambda_{\mathrm{adv}} \mathcal{L}_{\mathrm{adv}} + \lambda_{\mathrm{fm}} \mathcal{L}_{\mathrm{fm}} + \lambda_{\mathrm{rvq}} \mathcal{L}_{\mathrm{rvq}} + 
\lambda_{\mathrm{con}} \mathcal{L}_{\mathrm{consistency}}
$$
% 具体公式放附录 与本文提出的方法关系不大.

% \mathcal{L}_t(x, \hat{x}) = \| x - \hat{x} \|_1


% \begin{aligned}
% \mathcal{L}_{f}(x, \hat{x}) & =\frac{1}{|\alpha|} \sum_{i \in \alpha}\left(\left\|\mathcal{S}_{i}(x)-\mathcal{S}_{i}(\hat{x})\right\|_{1}+\left\|\mathcal{S}_{i}(x)-\mathcal{S}_{i}(\hat{x})\right\|_{2}\right. \\
% & \left.+\left\|\mathcal{M}_{i}(x)-\mathcal{M}_{i}(\hat{x})\right\|_{1}+\left\|\mathcal{M}_{i}(x)-\mathcal{M}_{i}(\hat{x})\right\|_{2}\right)
% \end{aligned}

% \mathcal{L}_{\text{adv}} (\hat{x}) = \mathbb{E}_{\hat{x}} \left[ \frac{1}{K} \sum_{k,t} \frac{1}{T_k} \max(0, 1 - D_{k, t}(\hat{x})) \right]

% \mathcal{L}_{\text{feat}} (x, \hat{x}) = \mathbb{E}_{x, \hat{x}} \left[ \frac{1}{KL} \sum_{k,t,l} \frac{1}{T_k} \left\| D^{(l)}_{k, t} (x) - D^{(l)}_{k, t} (\hat{x}) \right\|_1 \right]

% \mathcal{L}_{\text{cm}} = \| V - \text{RVQ}(V) \|_2 + \frac{1}{N} \sum_{i} \| Q_{i-1} - \text{VQ}(Q_{i-1}) \|_2

% \mathcal{L} = \lambda_{t} \mathcal{L}_{t} + \lambda_{f} \mathcal{L}_{f} + \lambda_{\text{adv}} \mathcal{L}_{\text{adv}} + \lambda_{\text{feat}} \mathcal{L}_{\text{feat}} + \lambda_{\text{cm}} \mathcal{L}_{\text{cm}}


==> section/3_method_zh.tex <==
3 Method

3.1 Overview

neural audio codec通过RVQ框架将连续的音频信号编码至离散的隐空间, 并量化得到一系列离散声学单元, 随后重构为原来的音频以实现音频压缩.  利用这些离散声学单元, 多种TTS模型和多模态LLM能够更有效的理解和生成音频. 然而, neural audio codec的一大挑战是一对多关系, 即相同的音频内容可能会被离散化成不同的声学表征, 从而加大了下游模型对离散声学单元的学习难度.

我们认为, 一个理想的neural audio codec, 应当规避"一对多"关系, 并保持声学表征的"一致性"特征. 这种一致性主要体现在两个方面: 1) 切片一致性: 具有相同内容的音频片段应被编码成一致的声学表示. 2) 扰动一致性: 在经过人耳难以察觉的微小扰动后, 音频信号的声学表征维持稳定不变. 通过维护这样的一致性, 生成的离散声学单元会表现出更高的规律性, 从而提升codec LM在预测浅层离散声学单元预测的准确率，并改善生成音频的内容真实性与说话人音色相似度。

在本章节中, 我们首先探讨neural audio codec内在的一对多关系, 以及对下游codec LM的潜在影响. 接着, 我们引入一致性准确率作为衡量一对多关系的指标. 紧随其后的，是对抑制一对多关系的一致性约束的详细介绍, 包括内容上的切片一致性和听感上的扰动一致性. 应用一致性约束旨在消除neural audio codec中的一对多关系，以增强codec LM对离散声学单元的预测准确率。

3.2 Neural audio codec

一段连续的音频信号可以表示为$X = \begin{bmatrix} x_{1,1} & \cdots & x_{1,T} \\ \vdots & \ddots & \vdots \\ x_{C,1} & \cdots & x_{C,T} \end{bmatrix} \in \mathbb{R}^{C \times T}$, 其中$C$表示音频通道的数量, 而$T$则代表帧数. neural audio codec通常由4个主要部分组成: encoder $E$, residual vector quantizer $Q$, decoder $G$和discriminator $D$ . 为简化讨论, 在本文中我们将音频的通道数量$C$简化为1, 但所述方法也同样适用于多声道音频。

在编码过程中, 首先, encoder从连续的音频信号$X^{T}$中提取特征, 将其编码成隐向量$Z^{\frac{T}{f_{ds}}}$, 这里$f_{ds}$表示encoder的下采样率. 接下来, quantizer根据欧式距离将$Z^{\frac{T}{f_{ds}}}$映射到最近的codebook embedding $C$上, 得到量化的$E^{\frac{T}{f_{ds}}}$. 最后, decoder从压缩后的$E^{\frac{T}{f_{ds}}}$中重建原始音频, 得到$\hat{X}$. 在训练阶段，为了减少重构音频与原始音频之间在人耳感知上的差异，discriminator 的任务是鉴别音频样本是原始的还是被重构的，通过这种监督方法来优化高频信号的再现质量。

3.3 Neural audio codec中的一对多关系

\begin{figure}
  \centering
  \includegraphics[width=.8\textwidth]{figure/model.jpg}
  \caption{model,草稿}
  \label{model}
\end{figure}


在本小节中, 我们构造一对含有相同内容的音频信号, 来探讨neural audio codec处理具有相同内容的音频信号时，是否会将其编码成不同的离散声学单元, 换言之, 一段音频是否会对应多种表征.

具体来说, 给定音频信号$X_1 = [x_1, \ldots, x_{t}]$, 我们通过选取$X_1$在时间区间$I_t = [t_s, t_e]$内的音频samples, 得到子音频片段$X_2 = [x_{t_s}, \ldots, x_{t_e}]$. 换言之, $X_2$ 是原始音频信号 $X_1$ 在该时间区间内的子序列。目的是对比这两段音频信号被编码后的差异。我们将这个操作称为在时域上的切片, 记为$S_t$, 即
$$X_2 = S_t(X_1) = \{x_i \mid x_i \in X_1, t_s \leq i \leq t_e\}$$
在neural audio codec中, encoder将$X_1$ 和$X_2$ 分别编码为隐向量$Z_1 = [z_1, \ldots, z_\frac{t}{f_{ds}}]$ 和$Z_2 = [z_\frac{t_s}{f_{ds}}, \ldots, z_\frac{t_e}{f_{ds}}]$. 然后, quantizer将这些隐向量量化为离散后声学单元序列$E_1 = [e_1, \ldots, e_\frac{t}{f_{ds}}]$ 和$E_2 = [e_\frac{t_s}{f_{ds}}, \ldots, e_\frac{t_e}{f_{ds}}]$. 所选取的audio samples在时间区间$I_t$内经过encoder $f_{ds}$倍下采样后, 对应的隐向量中的特征区间标记为$I_f = [\frac{t_s}{f_{ds}}, \frac{t_e}{f_{ds}}]$. 通过截取$Z_1$和$E_1$在特征区间$I_f$内的序列, 我们得到$\tilde{Z_1}$和$\tilde{E_1}$. 值得注意的是, 选取的音频区间的边界$t_s$和$t_e$是$f_{ds}$的整数倍, 以避免$Z_2$与$\tilde{Z_1}$之间发生时序上的偏移. 我们将这个操作称为在特征序列上的切片, 记为$S_f$, 即
$$\tilde{Z_1} = S_f(Z_1) = \{z_i \mid z_i \in Z_1, \frac{t_s}{f_{ds}} \leq i \leq \frac{t_e}{f_{ds}}\}$$
$$\tilde{E_1} = S_f(E_1) = \{e_i \mid e_i \in E_1, \frac{t_s}{f_{ds}} \leq i \leq \frac{t_e}{f_{ds}}\}$$
显然, $\tilde{Z_1}$和$Z_2$编码了相同的音频samples. 直观上, 我们期望经过quantizer处理后的离散声学表征$\tilde{E_1}$和$E_2$是相同的. 然而, encoder中卷积层的存在使$\tilde{Z_1}$捕捉到了感受野中其他的audio samples的特征. 此外, layer normalization或者time group normalization使得$\tilde{Z_1}$融合全局特征, 导致$\tilde{Z_1}$比$Z_2$包含了额外的音频信息. 因此, 尽管$\tilde{Z_1}$和$Z_2$编码了相同的音频内容, $\tilde{E_1}$和$E_2$却表现为差异显著, 产生了"一对多"关系, 即相同的音频内容, 编码后对应不同的声学表征, 这加大了下游codec LM的学习难度.

在codec LM中，精确预测前几层的离散声学单元序列非常关键。?发现，随着codebook层级的增加，codewords中携带的信息量逐渐减少。而RVQ中浅层的codewords包含了更多的语义和声学信息。因此，为了确保能够准确生成音频内容以及音色等副声学属性，codec LM至少需要准确预测浅层的离散声学单元序列。显而易见的是, 一对多关系会增加codec LM在预测浅层离散声学单元序列的难度, 影响WER和speaker timbre similarity等关键指标. 当neural audio codec维持声学表征的“一致性”时, 其生成的离散声学单元会表现出更加规律的内在特性, 从而提高codec LM在预测浅层离散声学单元的准确率。

3.4 一致性约束的策略

我们通过计算离散声学单元序列$\tilde{E_1}$和$E_2$之间的一致性来量化neural audio codec中“一对多”关系的程度，具体地，
$$acc_{\text{consistency}} = \frac{1}{T} \sum_{i=1}^{T} \mathbb{I}(\tilde{E}_1[i] = E_2[i]),$$
其中$T$是序列的长度，$\mathbb{I}\{\cdot\}$是指示函数，其值根据括号内的条件是否成立赋值为1或0，即若条件为真，则$\mathbb{I}(\cdot)=1$，否则$\mathbb{I}(\cdot)=0$。本文中的一致性度量$acc_{\text{consistency}}$与“一对多”关系呈负相关：一致性度量值越高，表示“一对多”问题越不显著；一致性度量值越低，则表明“一对多”关系越显著。关于neural audio codec中的“一对多”关系，我们将在后续章节进行详细分析。

根据第3.3节的分析，我们提出可以从以下两方面提升neural audio codec的一致性，以消除“一对多”关系：

1) 切片一致性：对于编码了相同音频内容的声学表征$\tilde{Z}_1$和$Z_2$，它们应当相同。因此，在通过量化器（quantizer）处理后，相应的离散声学单元序列$\tilde{E}_1$和$E_2$才能保持一致。为了迫使$\tilde{Z}_1$和$Z_2$达到一致性，我们使用均方误差（MSE）作为约束，即
$$loss_\text{slice} = \text{MSE}(\tilde{Z}_1, Z_2)$$

2) 扰动一致性：原始音频信号$X_1$经过人耳难以察觉的微小扰动$P$后得到的新音频信号$X^*_1$，在听感上应与$X_1$相似。微小扰动$P$可以通过不同的方法施加，例如添加在音频处理中不易被察觉的噪声或压缩，或通过在不显著改变波形结构的情况下微调音频信号的相位。由于人耳对相位直接感知能力有限，因此相位变化通常不易被感知。我们也使用MSE来约束受扰动前后的编码表征，即
$$X^*_1 = P(X_1)$$
$$loss_\text{perception} = \text{MSE}(E(X_1), E(X^*_1))$$

我们认为，理想的神经音频编解码器应满足切片一致性和扰动一致性，使得经过扰动后的表征$E(X^*_1)$在特定的特征区间$I_f = [\frac{t_s}{f_{ds}}, \frac{t_e}{f_{ds}}]$上与$Z_2$保持相同。具体来说，对于音频信号$X$，我们应用切片一致性和扰动一致性来约束它，即
$$loss_\text{consistency} = \text{MSE}(S_f \circ E \circ P(X), E \circ S_t \circ X)$$

==> section/4_experiment.tex <==
\subsection{Experimental Configuration}

%\textbf{Datasets}. We use approximately 44,000 hours of TTS datasets as training set, including LibriTTS~\citep{zen2019libritts} and large-scale MLS~\citep{PratapMLS} dataset. During the training process of neural audio codecs, each iteration randomly selects 20,480 audio samples from each audio segment. We then extract discrete units using neural audio codec and train VALL-E\citep{VALL-E}. For evaluation, we test the reconstructed audio of the neural audio codec and the speech generated by VALL-E on LibriTTS test set. We demonstrate the performance of VALL-E\citep{VALL-E}, using our codec as the audio tokenizer, trained on 960 hours and 44,000 hours of audio training data respectively.
\textbf{Datasets}. During the training process of neural audio codecs, we use LibriTTS~\citep{zen2019libritts} dataset, which comprises 960 hours of transcribed speech data, 
and we expand the dataset to 44,000 hours of large-scale MLS~\citep{PratapMLS} dataset to further validate the effectiveness of our method on large-scale data. We also employ our codec on VALL-E~\citep{VALL-E} to demonstrate the effectiveness of our approach for downstream TTS tasks. The test set of LibriTTS~\citep{zen2019libritts} is used as test data, which is randomly selected for 2,300 audio samples to verify the consistency of codecs and 500 audio samples to validate TTS performance.


%\textbf{Model}. We explore the impact of different consistency constraint strategies on the performance of the neural audio codec and downstream zero-shot TTS models. Specifically, we investigate the effect of adding slice consistency constraints, focusing on the length or proportion of the slice interval within the slicing operation $S_f$. For example, we explore extracting segments of varying proportions from $X_1$ and $E_1$ to obtain $X_2$ and $E_2$, aiming to determine which proportion yields better TTS model. We refer to this proportion as the \textbf{slice percentage}. Additionally, we test perceptual consistency by adding phase perturbations that are imperceptible to the human ear to the audio, and assess whether the codec can effectively reconstruct the audio after this \textbf{perturbation method}. We set the weight $\lambda_{con}$ for the consistency constraint loss function to 10.0.

\textbf{Training settings}. We train neural audio codecs for up to 350,000 iterations. During the training process of neural audio codecs, all audio samples are truncated to a fixed length of 1.28 seconds and resampled to 16 kHz with the batch size of 384. The codec is optimized by the Adam optimizer, with an initial learning rate of 3e-4 and beta parameters set to (0.5, 0.9). The reproducted VALL-E~\citep{VALL-E} is trained for 1,300k steps with the batch size of 56. The model is optimized by the Adam optimizer, with parameters $\beta$ = (0.9, 0.95). And we set the weight $\lambda_{con}$ for the consistency loss function to 10.0.

%\textbf{Neural audio codec baseline}. We adopt EnCodec~\citep{defossez2022high}, HiFiCodec~\citep{yang2023hifi}, FunCodec~\citep{du2024funcodec} and SpeechTokenize~r\citep{zhang2023speechtokenizer} as baseline models. To ensure fair comparison, we use the official open-source checkpoints for baseline neural audio codecs. We train our codec with consistency constraints, briefly calling it \textbf{ours}.
\textbf{Neural audio codec baseline}. To ensure fair comparison, we use the official open-source checkpoints from EnCodec~\citep{defossez2022high}, HiFiCodec~\citep{yang2023hifi}, FunCodec~\citep{du2024funcodec} and SpeechTokenizer~\citep{zhang2023speechtokenizer} as baseline models. And we train our codec with consistency loss, denoted as \textbf{ours}.

%We adopt EnCodec~\citep{defossez2022high}, HiFiCodec~\citep{yang2023hifi}, FunCodec~\citep{du2024funcodec} and SpeechTokenizer~\citep{zhang2023speechtokenizer} as baseline models. To ensure fair comparison, we use the official open-source checkpoints for baseline neural audio codecs. We train our codec with consistency constraints, briefly calling it \textbf{ours}.
% Since there is no official open-source version of VALL-E available, we use the open-source reproduction provided in FunCodec toolkit. 
% EnCodec is an advanced neural audio codec based on the RVQ framework.
% FunCodec is an open-source foundational neural audio codec toolkit that allows for the rapid construction of various neural audio codecs and the reproduction of neural codec language models like VALL-E. and build the proposed ConsistencyCodec based on FunCodec.


\textbf{Neural codec language model baseline}. We employ the SOTA neural codec language models as baselines, including SpeechGPT~\citep{zhang2023speechgpt}, SpeechTokenizer-based USLM~\citep{zhang2023speechtokenizer}, AnyGPT~\citep{zhan2024anygpt}, VoiceCraft~\citep{peng2024voicecraft}, XTTS v2~\citep{casanova2024xtts} and VALL-E~\citep{VALL-E} reproduced by Amphion~\citep{zhang2023amphion}. And we also use discrete audio tokens generated by our proposed methods to reproduce VALL-E~\citep{VALL-E} model which can help demonstrate the advantages of our methods. We provide more details about baseline neural codec language models in Appendix~\ref{appendix_baseline}.

%Please refer to \ref{appendix_baseline} for more details about baseline neural codec language models. 
% SpeechGPT, USLM, AnyGPT, VoiceCraft, XTTS_v2, VALL-E(amphion)

\subsection{Evaluation Metrics}

\subsubsection{Evaluation of Speech Reconstruction}

% \textbf{Objective evaluation}. 
We adopt consistency accuracy across all layers of neural audio codecs to measure the DRI phenomenon. Given that the codewords in the first few layers of the neural audio codec store most of the acoustic information, their consistency significantly affects the performance of downstream neural codec language models. Therefore, we especially present the first 3 layers' consistency accuracy. In addition, we also use ViSQOL~\citep{chinen2020visqol} and PESQ~\citep{rix2001perceptual} to measure the quality of the reconstructed speech~\citep{defossez2022high, zeghidour2021soundstream}. The higher scores of ViSQOL and PESQ indicate the better quality of audio.

 %Following the settings of EnCodec~\citep{defossez2022high, } and SoundStream~\citep{zeghidour2021soundstream},

% \textbf{Subjective evaluation}.

\subsubsection{Evaluation of Speech Generation}
%We use WER, speaker similarity and UTMOS~\citep{saeki2022utmos} to evaluate the speech quality of neural codec language models. 
\textbf{Objective evaluation}. We use the Whisper~\citep{radford2023robust} model to transcribe the generated speech and calculate the WER. To evaluate speaker similarity, we first use 3D-speaker~\citep{chen20243d} toolkit to extract speaker embeddings from the generated speech and reference speech, and then compute the cosine similarity between the normalized embeddings. We also employ UTMOS~\citep{saeki2022utmos} as an automatic MOS prediction system to assess the naturalness of the speech.
% WER measures the content accuracy of the generated speech, and speaker similarity assesses the resemblance in timbre between the generated speech and the prompt speech.

\textbf{Subjective evaluation}. We randomly select 50 audio samples from the LibriTTS~\citep{zen2019libritts} test set to conduct MOS and SMOS test. MOS assesses the naturalness of the generated speech, while SMOS measures the similarity between the generated speech and the original speaker's voice. Both MOS and SMOS range from 1 to 5, with higher values indicating better speech quality and greater voice similarity.



==> section/4_result_analysis.tex <==
In this section, we evaluate the effectiveness of slice-consistency and perturbation-consistency methods. Firstly, We compare the speech reconstruction results of the neural audio codec based on our method and baseline models. And then we demonstrate that introducing our approach to TTS model like VALL-E~\citep{VALL-E} can effectively enhance speech generation performance on both small-scale and large-scale data. Finally, we conduct ablation studies to illustrate the effects of the slice-consistency and perturbation-consistency methods during training, respectively.

%In this section, we first validate the effectiveness of the consistency constraint on the neural audio codec, and then use the codec as an audio tokenizer for training the VALL-E~\citep{VALL-E} model. We expand the TTS corpus from 960 hours to 44K hours and find that, training on large-scale dataset, the consistency constraint can still reduce the DRI phenomenon and effectively enhance the speech generation capability of the downstream neural codec language model. Finally, we explore the roles of slice-consistency and perturbation-consistency in the consistency constraint methods through ablation study.


\subsection{Speech Reconstruction Results}
%The codebook size of all codecs is set to 1024. The consistency constraint strategy involves setting the slice percentage to 20\% and applying phase perturbation. 
\begin{table}
    \centering
    \caption{The speech reconstruction results on LibriTTS test set. \textbf{Bold} means the best result, and \underline{underline} means the second-best result.}
    \scalebox{0.83}{
    \begin{tabular}{c|ccc|cccc}
    \toprule
    \multirow{2}{*}{\makecell[c]{Neural\\Audio Codec}} & \multirow{2}{*}{\makecell[c]{Sampling\\Rate}} & \multirow{2}{*}{\makecell[c]{Number of\\Codebooks}} & \multirow{2}{*}{Bandwidth} & \multirow{2}{*}{Consistency↑} & \multirow{2}{*}{\makecell[c]{First 3 Layers'\\Consistency↑}} & \multirow{2}{*}{ViSQOL↑} & \multirow{2}{*}{PESQ↑} \\
    & & & & & & &
    \\ \midrule
    \multirow{3}{*}{EnCodec} & \multirow{3}{*}{24kHz} & 8 & 6.0 kbps & \underline{69.00\%} & 83.71\% & 4.35 & 2.73 \\
    & & 16 & 12.0 kbps & 51.18\% & 83.71\% & 4.52 & 3.35 \\
    & & 32 & 24.0 kbps & 30.19\% & 83.71\% & \underline{4.60} & \textbf{3.67} \\ 
    \midrule
    \multirow{2}{*}{HiFiCodec} & 16kHz & 4 & 2.0 kbps & 59.28\% & 65.14\% & 4.31 & 2.81 \\
    & 24kHz & 4 & 3.0 kbps & 57.92\% & 64.44\% & 4.32 & 2.76 \\ \midrule
    SpeechTokenizer & 16kHz & 8 & 4.0 kbps & 30.51\% & 51.26\% & 4.36 & 2.62 \\
    \midrule
    \multirow{2}{*}{FunCodec} & \multirow{2}{*}{16kHz} & 8 & 4.0 kbps & 12.21\% & 24.80\% & 4.47 & 3.26 \\
    & & 16 & 8.0 kbps & 6.43\% & 22.35\% & 4.57 & \underline{3.62} \\ \midrule
    \multirow{2}{*}{Ours} & \multirow{2}{*}{16kHz} & 8 & 4.0 kbps & \textbf{80.75\%} & \underline{93.98\%} & 4.45 & 3.25 \\ 
    & & 16 & 8.0 kbps & 66.65\% & \textbf{95.38\%} & \textbf{4.64} & 3.59 \\
    \bottomrule
    \end{tabular}
    }
    \label{codec}
\end{table}


 
We evaluate the effectiveness of our method from the perspective of consistency and reconstructed speech quality. First, we compare the consistency accuracy between the neural audio codec based on our method and baseline models. The results presented in Table~\ref{codec} demonstrate that the neural audio codec based on our method can reconstruct speech with superior consistency accuracy compared to baseline systems, achieving the rate of 80.75\% across all layers and the rate of 95.38\% in the first 3 layers. In contrast, the baseline models 
suffer from low consistency accuracy, indicating that the same audio segments are encoded into different discrete audio tokens. We also observe that consistency accuracy of all layers outperforms that of the the first 3 layers, particularly in baseline models, which increases the difficulty for downstream neural codec language models in predicting the codewords from deeper layers. Then we evaluate ViSQOL~\citep{chinen2020visqol} and PESQ~\citep{rix2001perceptual} to evaluate the reconstructed speech quality. The results in Table~\ref{codec} show that the ViSQOL~\citep{chinen2020visqol} of the neural audio codec based on our method surpasses all baseline models, achieving a score of 4.64. Additionally, the PESQ~\citep{rix2001perceptual} is also comparable to that of the baseline models.   This suggests that our method can be confidently applied to neural audio codecs without negatively impacting reconstruction performance.
 

%Table~\ref{codec} presents the audio reconstruction results of various neural audio codecs. Considering that neural codec language models typically employs the first 8 quantizers of the codec to discretize speech, Table \ref{every_layer_consistency} shows the consistency accuracy of the first 8 layers for each codec. Here are our observations:

%1. Popular neural audio codecs, including EnCodec~\citep{defossez2022high} and HiFiCodec~\citep{yang2023hifi}, suffer from low consistency accuracy, indicating that the same audio segments are encoded into different discrete units. As shown in Table ~\ref{every_layer_consistency}, the consistency accuracy at deeper layer in EnCodec drops sharply from 90.57\% to 49.41\%. This illustrates that the correspondence between audio segments and codewords in deeper layer becomes more ambiguous, which increases the difficulty for downstream neural codec language models to predict deeper layer codewords.

%2. Compared to baseline neural audio codecs, ours exhibits a significant improvement in the consistency accuracy across all layers, especially in the first 3 layers. Moreover, its reconstruction capability remains unaffected and even shows a slight improvement in the ViSQOL metric, increasing by 0.07. This indicates that consistency constraints can be confidently applied to neural audio codecs without worrying about a decline in reconstruction performance.

% 3. The reconstruction results of EnCodec is inferior to that of FunCodec and ConsistencyCodec. EnCodec with 32 codebooks barely outperforms FunCodec and ConsistencyCodec with only 16 codebooks (model id 3 vs. model id 16). Therefore, for downstream zero-shot TTS tasks, we choose FunCodec and ConsistencyCodec to discretize speech.



\subsection{Speech Generation Results}

% \begin{table}[!ht]
%     \centering
%     \caption{The zero-shot TTS evaluation results for VALL-E trained on LibriTTS. \textbf{Bold} for the best result, and \underline{underline} for the second-best result.}
%     \scalebox{0.9}{
%     \begin{tabular}{c|cccc|ccc}
%         \toprule
%         \multirow{3}{*}{id} & \multicolumn{4}{c|}{codec model} & \multicolumn{3}{c}{TTS model} \\
%         \cline{2-8}
%         & slice & perturb method & consistency↑ & \makecell[c]{first 3 layers'\\consistency↑} & WER↓ & SIM↑ & UTMOS↑ \\
%         \midrule
%         1 & / & / & 11.87\% & 23.92\% & 13.11 & 79.61\% & 4.12 \\
%         \midrule
%         2 & 20\% & phase perturb & \textbf{86.38\%} & \textbf{95.77\%} & \textbf{6.90} & \textbf{86.92\%} & \textbf{4.32} \\
%         \midrule
%         3 & 40\% & phase perturb & 76.05\% & 91.44\% & \underline{8.01} & \underline{84.42\%} & \underline{4.30} \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:valle_960}
% \end{table}


% \begin{table}[!ht]
%     \centering
%     \caption{Consistency accuracy of ConsistencyCodec at different slice percentages.}
%     \scalebox{1.0}{
%     \begin{tabular}{c c c c}
%         \toprule
%         slice percentage & consistency & first 3 layers's consistency & last 3 layers's consistency \\ 
%         \midrule
%         20\% & 78.65\% & 92.38\% & 64.93\% \\ 
%         40\% & 82.47\% & 93.89\% & 70.66\% \\ 
%         60\% & 84.44\% & 95.00\% & 73.33\% \\ 
%         80\% & 85.48\% & 95.44\% & 75.02\% \\ 
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:various_slice_percentage}
% \end{table}


% \subsection{Effectiveness of Data Scaling}


% \begin{table}
%     \centering
%     \caption{The speech generation evaluation on LibriTTS test set. \textbf{Bold} means the best result, and \underline{underline} means the second-best result.}
%     \scalebox{0.95}{
%     \begin{tabular}{c|cc|ccc}
%     \toprule
%         % Neural Audio Codec & Neural Codec Language Model & Bandwidth & WER↓ & SIM↑ & UTMOS↑ \\
%         \multirow{2}{*}{Neural Audio Codec} & \multirow{2}{*}{\makecell[c]{Neural Codec\\ Language Model}} & \multirow{2}{*}{Bandwidth} & \multirow{2}{*}{WER↓} & \multirow{2}{*}{SIM↑} & \multirow{2}{*}{UTMOS↑} \\ 
%          & & & & & \\ \midrule
%         % \multicolumn{4}{c|}{Ground Truth} & 0.0 & 100.0\% & 4.16 \\
%     % \midrule
%         mHuBERT & SpeechGPT_{72Kh}\footnote{\url{https://huggingface.co/fnlp/SpeechGPT-7B-com}} & 0.5 kbps & 22.41 & 15.70\% & \underline{4.08} \\ 
%     \midrule
%         \multirow{2}{*}{EnCodec} & VoiceCraft_{330M,9Kh}\footnote{\url{https://huggingface.co/pyp1/VoiceCraft_giga330M}} & \multirow{2}{*}{2.2 kbps} & 6.92 & 74.99\% & 3.54 \\ 
%          & VoiceCraft_{830M,9Kh}\footnote{\url{https://huggingface.co/pyp1/VoiceCraft_830M_TTSEnhanced}} & & 6.07 & 81.21\% & 3.81 \\ 
%     \midrule
%         Mel VQ-VAE & XTTS v2_{27Kh}\footnote{\url{https://huggingface.co/coqui/XTTS-v2}} & / & \underline{4.38} & \textbf{88.57\%} & 3.93 \\ 
%     \midrule
%         \multirow{3}{*}{SpeechTokenizer} & USLM_{960h}\footnote{\url{https://huggingface.co/fnlp/USLM}} & \multirow{3}{*}{4.0 kbps} & 15.78 & 47.60\% & 3.09 \\ 
%         & AnyGPT_{57Kh}\footnote{\url{https://huggingface.co/fnlp/AnyGPT-chat}} & & 28.22 & 35.60\% & 3.16 \\ 
%         & VALL-E_{960h}\footnote{\url{https://github.com/open-mmlab/Amphion/tree/main/egs/tts/VALLE_V2}} & & 5.00 & 81.77\% & 4.03 \\ 
%     \midrule
%         \multirow{2}{*}{\makecell[c]{Ours w/o\\consistency loss}} & VALL-E_{960h} & \multirow{2}{*}{4.0 kbps} & 13.11 & 76.91\% & 4.12 \\ 
%         & VALL-E_{44Kh} &  & 5.51 & 83.58\% & 4.13 \\
%     \midrule
%         \multirow{2}{*}{Ours} & VALL-E_{960h} & \multirow{2}{*}{4.0 kbps} & 6.90 & 86.92\% & \textbf{4.32} \\ 
%         & VALL-E_{44Kh} &  & \textbf{3.85} & \underline{87.24\%} & \textbf{4.32} \\
%         % Ours & VALL-E & 4.0 kbps & \textbf{3.85} & \underline{87.24\%} & \textbf{4.32} \\ 
%     \bottomrule
%     \end{tabular}
%     }
%     \label{tts}
% \end{table}


\begin{table}
    \centering
    \caption{The speech generation evaluation on LibriTTS test set. \textbf{Bold} means the best result, and \underline{underline} means the second-best result.}
    \scalebox{0.95}{
    \begin{tabular}{c|cc|ccc}
    \toprule
        % Neural Audio Codec & Neural Codec Language Model & Bandwidth & WER↓ & SIM↑ & UTMOS↑ \\
        \multirow{2}{*}{Neural Audio Codec} & \multirow{2}{*}{\makecell[c]{Neural Codec\\ Language Model}} & \multirow{2}{*}{Bandwidth} & \multirow{2}{*}{WER↓} & \multirow{2}{*}{UTMOS↑} & \multirow{2}{*}{SIM↑} \\ 
         & & & & & \\ \midrule
        % \multicolumn{4}{c|}{Ground Truth} & 0.0 & 100.0\% & 4.16 \\
    % \midrule
        mHuBERT & SpeechGPT_{72Kh}\footnote{\url{https://huggingface.co/fnlp/SpeechGPT-7B-com}} & 0.5 kbps & 22.41 & \underline{4.08} & 15.70\% \\ 
    \midrule
        \multirow{2}{*}{EnCodec} & VoiceCraft_{330M,9Kh}\footnote{\url{https://huggingface.co/pyp1/VoiceCraft_giga330M}} & \multirow{2}{*}{2.2 kbps} & 6.92 & 3.54 & 74.99\% \\ 
         & VoiceCraft_{830M,9Kh}\footnote{\url{https://huggingface.co/pyp1/VoiceCraft_830M_TTSEnhanced}} & & 6.07 & 3.81 & 81.21\% \\ 
    \midrule
        Mel VQ-VAE & XTTS v2_{27Kh}\footnote{\url{https://huggingface.co/coqui/XTTS-v2}} & / & \underline{4.38} & 3.93 & \textbf{88.57\%} \\ 
    \midrule
        \multirow{3}{*}{SpeechTokenizer} & USLM_{960h}\footnote{\url{https://huggingface.co/fnlp/USLM}} & \multirow{3}{*}{4.0 kbps} & 15.78 & 3.09 & 47.60\% \\ 
        & AnyGPT_{57Kh}\footnote{\url{https://huggingface.co/fnlp/AnyGPT-chat}} & & 28.22 & 3.16 & 35.60\% \\ 
        & VALL-E_{960h}\footnote{\url{https://github.com/open-mmlab/Amphion/tree/main/egs/tts/VALLE_V2}} & & 5.00 & 4.03 & 81.77\% \\ 
    \midrule
        \multirow{2}{*}{\makecell[c]{Ours w/o\\consistency loss}} & VALL-E_{960h} & \multirow{2}{*}{4.0 kbps} & 13.11 & 4.12 & 76.91\% \\ 
        & VALL-E_{44Kh} &  & 5.51 & 4.13 & 83.58\% \\
    \midrule
        \multirow{2}{*}{Ours} & VALL-E_{960h} & \multirow{2}{*}{4.0 kbps} & 6.90 & \textbf{4.32} & 86.92\% \\ 
        & VALL-E_{44Kh} &  & \textbf{3.85} & \textbf{4.32} & \underline{87.24\%} \\
        % Ours & VALL-E & 4.0 kbps & \textbf{3.85} & \underline{87.24\%} & \textbf{4.32} \\ 
    \bottomrule
    \end{tabular}
    }
    \label{tts}
\end{table}

In this section, we employ the codec based on our method to reproduce VALL-E~\citep{VALL-E} and evaluate the generated speech from both subjective and objective perspectives to demonstrate the effectiveness of our method for downstream TTS tasks. Furthermore, we increase the training data from 960 hours of LibriTTS~\cite{zen2019libritts} to 44,000 hours of large-scale MLS~\citep{PratapMLS} dataset  to verify that our method is equally effective on large scale datasets.

\textbf{Subjective Evaluation}. According to the Table~\ref{tts}, we have the following observation: (1) VALL-E~\citep{VALL-E} trained by large-scale MLS~\citep{PratapMLS} dataset  with 
consistency loss outperforms all other baseline models on WER


\textbf{Effectiveness of consistency constraint methods}. Table \ref{tts} presents that the VALL-E~\citep{VALL-E} model achieves better results in WER, SIM and UTMOS compared to the VALL-E without the consistency constraint. This indicates that the generated speech exhibits superior intelligibility, speaker similarity and naturalness. Thus, it validates the effectiveness of the proposed consistency constraint method, which includes slice consistency and perturbation consistency. We explore optimal parameters of consistency constraint method, as shown in Table ~\ref{tab:valle_44kh} in the appendix.

% \textbf{Effectiveness of consistency constraint methods}. Table \ref{tts} presents that the VALL-E model, which trained on 44K hours, generates the best result when the slice percentage is 20\% with phase perturbation. Under these conditions, metrics such as WER, SIM, and UTMOS reach better values than other, indicating that the generated speech exhibits the best intelligibility, speaker similarity, and naturalness. This validates the effectiveness of the proposed consistency constraint method, including slice consistency and perturbation consistency.

\textbf{Extend to scalable data}. When the consistency constraint is applied and our codec is taken as the audio tokenizer, VALL-E trained on 44K hours demonstrates superior speech generation results compared to that trained on 960 hours, with WER dropping from 6.90 to 3.85 and speaker similarity increasing by 0.32\%. This confirms that the model with the consistency constraint benefits significantly from large-scale data.

\textbf{Compared with neural codec language models}. As shown in Table \ref{tts}, our proposed codec outperforms in terms of WER and UTMOS metrics, which indicates ours can generate high-quality and natural speech. Although our codec achieves a slightly lower SIM than XTTS v2 by 1.33\%, it significantly outperforms USLM and VALL-E (take SpeechTokenizer as The audio tokenizer) with similar architectures. This result confirms the effectiveness of the proposed consistency constraint.


\subsection{Ablation Study}


% \begin{table}[!ht]
%     \centering
%     \caption{Ablation experiments of different slices and perturb methods.}
%     \scalebox{1.0}{
%     \begin{tabular}{c|cc|c|c|c}
%     \toprule
%     \multirow{2}{*}{id} & \multicolumn{2}{c|}{codec config} & \multirow{2}{*}{WER↓} & \multirow{2}{*}{SIM↑} & \multirow{2}{*}{UTMOS↑} \\ \cline{2-3}\rule{0pt}{10pt}
%      & slice & perturb method &  &  &  \\ 
%     \midrule
%     1 & \multirow{2}{*}{/} & / & 13.12 & 78.02\% & 4.12 \\
%     2 &  & phase perturb & 11.09 & 77.18\% & 4.15 \\ \midrule
%     3 & \multirow{2}{*}{20\%} & / & 8.77 & 82.55\% & 4.16 \\
%     4 &  & phase perturb & \textbf{7.48} & \textbf{84.39\%} & \textbf{4.32} \\
%     \midrule
%     5 & \multirow{2}{*}{40\%} & / & 8.30 & \underline{83.62\%} & 4.20 \\
%     6 &  & phase perturb & \underline{7.66} & 83.13\% & \underline{4.29} \\
%     \midrule
%     7 & 0.1s & phase perturb & 8.79 & 81.64\% & 4.14 \\
%     8 & 0.3s & phase perturb & 8.92 & 81.31\% & 4.12 \\
%     \bottomrule
%     \end{tabular}
%     }
%     \label{ablation}
% \end{table}


% \makecell[c]{first 3 layers'\\consistency↑}

\begin{table}
    \centering
    \caption{Ablation study on slice consistency and perturbation consistency. \textbf{Bold} for the best result, and \underline{underline} for the second-best result.}
    \scalebox{1.0}{
    \begin{tabular}{cc|cc|ccc}
        \toprule
        \multicolumn{4}{c|}{\multirow{2}{*}{Neural Audio Codec}} & \multicolumn{3}{c}{\multirow{2}{*}{Neural Codec Language Model}} \\ 
        & \multicolumn{1}{c}{} & & & & & \\
        \cline{1-7}\rule{0pt}{16pt}
        Slice & Perturb Method & Consistency↑ & \makecell[c]{First 3 Layers'\\Consistency↑} & WER↓ & SIM↑ & UTMOS↑  \\
        \midrule
        \multirow{2}{*}{/} & / & 11.87\% & 23.92\% & 13.11 & 79.61\% & 4.12 \\ % \cmidrule{3-8}
         & phase perturb & 11.55\% & 23.19\% & 11.12 & 78.85\% & 4.12 \\
        \midrule
        0.1s & phase perturb & \underline{85.19\%} & \underline{95.22\%} & 8.11 & 83.21\% & 4.18 \\
        0.3s & phase perturb & 82.89\% & 93.85\% & 13.21 & 83.94\% & 4.16 \\
        \midrule
        \multirow{2}{*}{20\%} & / & 84.44\% & 94.63\% & 9.13 & 83.77\% & 4.15 \\ %\cmidrule{3-8}
         & phase perturb & \textbf{86.38\%} & \textbf{95.77\%} & \textbf{6.90} & \textbf{86.92\%} & \textbf{4.32} \\  
        \midrule
        \multirow{2}{*}{40\%} & / & 74.78\% & 90.92\% & 9.28 & \underline{84.91\%} & 4.22 \\ % \cmidrule{3-8}
         & phase perturb & 76.05\% & 91.44\% & \underline{8.01} & 84.42\% & \underline{4.30} \\       
        \bottomrule
    \end{tabular}
    }
    \label{ablation}
\end{table}

We conduct ablation studies on the prompt generation pipeline. First, we remove the design of the placeholder from the pipeline. In this case, LLM is required to directly write text prompts for each class in attributes, after which sentence combination is performed. The results are presented as ``- Placeholder'' in Table~\ref{ablation of prompt generation}. The drop in classification accuracy demonstrates that the placeholder is beneficial for the prompt generation pipeline. Without it, LLM might miss attributes or even alter them during sentence combination, resulting in low-quality text prompts. In addition to the placeholder, we also conduct ablation studies on instructing LLM to write only phrases or sentences by removing sentences (``- Sentence'') or phrases (``- Phrase''). The results indicate that variations in format can marginally improve the robustness of the prompt generation pipeline.

In this subsection, we conduct ablation experiments to verify the roles of slice consistency and perturbation consistency. After training neural audio codec with various configurations, we extract discrete units from the LibriTTS 960h dataset through these codecs and subsequently train VALL-E~\citep{VALL-E} on these units. The results are presented in Table \ref{ablation}. In the table, \textbf{slice} and \textbf{perturb method} represent slice consistency and perturbation consistency, respectively. The percentage in the slice column (e.g., 20\%) indicates the proportion of audio $X_1$ used to generate $X_2$, where the length of $X_2$ is variable; whereas the duration (e.g., 0.1s) refers to extracting a fixed duration from $X_1$ to create $X_2$. We observe that improving consistency accuracy generally leads to better TTS results.

1) When only perturbation consistency is applied, WER significantly decreases from 13.11 to 11.12, but speaker similarity does not improve. Although perturbation consistency does not enhance the consistency accuracy of the codec model, it improves the model’s generalization ability, allowing it to generate high-fidelity speech even when the discrete units are slightly perturbed, thus reducing the WER. 
% In the VALL-E model, prompt audio is discretized into discrete units to characterize the speaker's timbre. If the model’s consistency accuracy is low, it cannot effectively extract the speaker’s timbre from the discrete units, explaining the reason why speaker similarity does not improve when only perturbation consistency is applied.

2) When only slice consistency is employed, the consistency accuracy of the codec model increases significantly, and the TTS model’s WER and SIM also show marked improvement. This indicates that reducing the DRI phenomenon in the codec enhances the intelligibility and speaker's timbre similarity of the VALL-E~\citep{VALL-E} model. When either perturbation consistency or slice consistency is adopted, the VALL-E model generates higher-quality audio, validating the efficacy of the consistency constraints.

3) In slice consistency, the model with dynamic slice percentage (e.g., 20\%) performs better than the model with fixed slice interval (e.g., 0.1s). When using a slice percentage instead of a fixed duration, the length of the slice is dynamically adjusted relative to the entire audio sequence, which better accommodates audio segments of varying lengths.

4) Smaller slice length enhances TTS results. The VALL-E~\citep{VALL-E} model with a slice percentage of 20\% outperforms the model with a slice percentage of 40\%. The reason is that a smaller slice percentage (e.g., 20\%) extracts shorter audio segments, requiring the codec to encode with less contextual information. This reduces the DRI phenomenon and improves the consistency accuracy, leads to better performance of downstream VALL-E model.

==> section/5_related_work.tex <==
\textbf{Discrete speech representations}. Discrete speech representations can be categorized into discrete semantic units and discrete acoustic units. Discrete semantic units are extracted from self-supervised speech models like HuBERT\citep{hsu2021hubert} and WavLM\citep{Chen2021WavLM}, or ASR models like SenseVoice\citep{speechteam2024funaudiollm}. K-means or VQ models serve as information bottlenecks, filtering out paralinguistic information while retaining semantic information. In contrast, discrete acoustic units are encoded by neural audio codecs, preserving complete acoustic information and aiming to reconstruct high-fidelity audio. SoundStream\citep{zeghidour2021soundstream} and EnCodec\citep{defossez2022high} adopt RVQ framework to encode speech into multi-level discrete acoustic units. SingleCodec\citep{li2024single} and Disen-TF-Codec\citep{jiang2023disentangled} utilize a reference encoder to capture global time-invariant information, thereby reducing the number of codebooks. SpeechTokenize\citep{zhang2023speechtokenizer}, and FACodec\citep{ju2024naturalspeech} decouple speech into different attributes, making discrete units more suitable for downstream speech modeling tasks. We focus on modeling general speech, and conduct experiments on neural audio codec and discrete acoustic units.
% Neural codec language models, build upon discrete speech representations, demonstrate impressive capabilities in speech generation. 
% FreqCodec\citep{du2024funcodec} focuses on encoding the spectral features rather than raw audio; after filtering out high-frequency information, it achieves comparable performance with fewer parameters.


\textbf{Audio tokenizers and neural codec language models}. After tokenizing continuous audio signals into discrete units by a neural audio codec, a neural codec language model can be trained on these discrete units. VALL-E\citep{VALL-E} and SpearTTS\citep{kharitonov2023speak} employ EnCodec\citep{defossez2022high} and SoundStream\citep{zeghidour2021soundstream} as audio tokenizers to extract discrete acoustic units, aiming to retain all acoustic information. SpearTTS\citep{kharitonov2023speak} and SoundStorm\citep{borsos2023soundstorm} adopt a coarse-to-fine approach to generate discrete acoustic units. VoiceCraft\citep{peng2024voicecraft} rearrange audio tokens through an auto-regressive way to perform speech generation and editing tasks. LLM-Codec\citep{yang2024uniaudio} represent audio tokens with words or subwords from the vocabulary of LLMs, aligning audio modality with text modality. However, previous work\citep{yang2024uniaudio} noticed that even when audio segments contain the same sound events, the discrete units generated by the audio tokenizer may still exhibit inconsistencies. In this paper, we delve into this phenomenon, and propose consistency constraint method to mitigate it.

% This suggests that audio tokenizers may experience the phenomenon of \textbf{Discrete Representation Inconsistency (DRI)}, complicating the modeling of speech for these neural codec language models. 
% Early research\citep{lakhotia2021generative}\citep{lee2021textless}\citep{kharitonov2022textless} utilizes pre-trained SSL speech models, such as HuBERT\citep{hsu2021hubert} and WavLM\citep{Chen2021WavLM}, as audio tokenizers to extract discrete semantic units to build spoken language models. These models are effective in preserving and generating semantic information, but they overlook paralinguistic details like timbre and prosody. In contrast, 
% LanguageCodec\citep{ji2024language} improves the representation of deeper discrete acoustic units by limiting the number of channels in the top three layers of its codebook, enabling the neural codec language model to predict codewords more accurately. MobileSpeech\citep{ji2024mobilespeech} adopts a fully non-autoregressive way for predicting discrete units, thus speeding up the codec decoding process. VoiceCraft\citep{peng2024voicecraft} rearrange audio tokens through an auto-regressive way to perform speech generation and editing tasks. RALL-E\citep{xin2024rall} utilizes chain-of-thought prompting to decompose TTS tasks into simpler steps, thereby enhancing the robustness of LLM-based TTS. LLM-Codec\citep{yang2024uniaudio} represent audio tokens with words or subwords from the vocabulary of LLMs, aligning audio modality with text modality. However, UniAudio 1.5\citep{yang2024uniaudio} observes that even when audio segments contain the same sound events, the discrete units generated by the audio tokenizer may still exhibit inconsistencies. This suggests that audio tokenizers may experience the phenomenon of \textbf{Discrete Representation Inconsistency (DRI)}, complicating the modeling of speech for these neural codec language models.


% 其他codec的工作: semantic token, acoustic token. 更加关注general 的audio的表征，因此本文针对acoustic tokens 进行研究。
% UniAudio1.5也注意到了这种不一致的问题.

==> section/6_conclusion.tex <==
In this paper, we conduct a detailed analysis of the DRI phenomenon within audio tokenizers, and propose consistency constraints to mitigate this phenomenon, thereby enhancing the consistency between audio samples and discrete units: 1) Slice Consistency: ensuring that identical audio samples are encoded into consistent acoustic representations; 2) Perturbation Consistency: maintaining the acoustic representation of audio signals invariant under perturbations that are imperceptible to human ears. By applying consistency constraints to neural audio codecs, the neural codec language model outperforms SOTA TTS systems, generating higher quality speech and validating the effectiveness of the proposed consistency constraints.


==> section/demo.tex <==
123
